Entity6K: A Large Open-Domain Evaluation Dataset for Real-World Entity Recognition

Open-domain real-world entity recognition is essential yet challenging, involving identifying various entities in diverse environments. The lack of a suitable evaluation dataset has been a major obstacle in this field due to the vast number of entities and the extensive human effort required for data curation. We introduce Entity6K, a comprehensive dataset for real-world entity recognition, featuring 5,700 entities across 26 categories, each supported by 5 human-verified images with annotations. Entity6K offers a diverse range of entity names and categorizations, addressing a gap in existing datasets. We conducted benchmarks with existing models on tasks like image captioning, object detection, zero-shot classification, and dense captioning to demonstrate Entity6K's effectiveness in evaluating models' entity recognition capabilities. We believe Entity6K will be a valuable resource for advancing accurate entity recognition in open-domain settings.

==> tables/results_VQA.tex <==
\begin{tabular}{l|cccccccccccc} 
\toprule
\multirow{2}{*}{Methods}   & \multicolumn{8}{c}{Text Metrics} &\multicolumn{2}{c}{Accuracy}   \\ 
\cmidrule(r){2-9}\cmidrule(r){10-11} 
& ROUGE-1 & ROUGE-2 & ROUGE-L & BLEU $\uparrow$ & METEOR $\uparrow$ & CIDEr $\uparrow$ & SPICE $\uparrow$ &BertScore $\uparrow$ &Acc-full $\uparrow$ &Acc-part $\uparrow$  \\ 
\midrule
ViLT    \\ 
BLIP-base \\
BLIP-capfilt-large \\
GIT-base \\
GIT-large \\
PromptCap \\
\bottomrule
\end{tabular}

==> tables/results_VQA_specific.tex <==
\begin{tabular}{l|cccccccccccc} 
\toprule
\multirow{2}{*}{Methods}   & \multicolumn{8}{c}{Text Metrics} &\multicolumn{2}{c}{Accuracy}   \\ 
\cmidrule(r){2-9}\cmidrule(r){10-11} 
& ROUGE-1 & ROUGE-2 & ROUGE-L & BLEU $\uparrow$ & METEOR $\uparrow$ & CIDEr $\uparrow$ & SPICE $\uparrow$ &BertScore $\uparrow$ &Acc-full $\uparrow$ &Acc-part $\uparrow$  \\ 
\midrule
ViLT    \\ 
BLIP-base \\
BLIP-capfilt-large \\
GIT-base \\
GIT-large \\
PromptCap \\
\bottomrule
\end{tabular}

==> tables/results_captioning.tex <==
\begin{tabular}{l|rrrrrrr} 
\toprule
Methods   & ROUGE-1 $\uparrow$ & ROUGE-2 $\uparrow$ & ROUGE-L $\uparrow$ & BLEU $\uparrow$ & METEOR $\uparrow$ & SPICE $\uparrow$ & BertScore $\uparrow$  \\ 
\midrule
GRIT~\cite{Nguyen2022GRITFA} & 0.12 & 0 & 0.01 & 0.01 & 0.20 & 0.13 & 77.85 \\
GIT~\citep{Wang2022GITAG} & 11.32 & 1.11 & 9.92 & 0.40 & 4.37  & 1.27 & 81.34 \\
BLIP~\citep{Li2022BLIPBL} & \textbf{13.83} & 0.82 & 11.67 & \textbf{1.11} & \textbf{7.75}  & 1.74 & 84.52 \\
OFA~\citep{Wang2022UnifyingAT} & 13.54 & \textbf{2.16} & \textbf{12.02} & 0.92 & 6.89  & \textbf{3.27} & \textbf{84.63} \\
%GPT-4 \\
\bottomrule
\end{tabular}


